On the free-precession candidate PSR B1828-11: Evidence for increasing deformation

We observe that the periodic variations in spin-down rate and beam-width of the radio pulsar PSR B1828-11 are getting faster. In the context of a free precession model, this corresponds to a decrease in the precession period $P_{\mathrm{fp}}$. We investigate how a precession model can account for such a decrease in $P_{\mathrm{fp}}$, in terms of an increase over time in the absolute biaxial deformation ($|\epsilon_{\mathrm{p}}|{\sim}10^{-8}$) of this pulsar. We perform a Bayesian model comparison against the 'base' precession model (with constant $\epsilon_{\mathrm{p}}$) developed in Ashton et al (2016), and we obtain decisive odds in favour of a time-varying deformation. We study two types of time-variation: (i) a linear drift with a posterior estimate of $\dot{\epsilon}_{\mathrm{p}}{\sim}10^{-18}\,\mathrm{s}^{-1}$ and odds of $10^{75}$ compared to the base-model, and (ii) $N$ discrete positive jumps in $\epsilon_{\mathrm{p}}$ with very similar odds to the linear $\epsilon_{\mathrm{p}}$-drift model. The physical mechanism explaining this behaviour is unclear, but the observation could provide a crucial probe of the interior physics of neutron stars. We also place an upper bound on the rate at which the precessional motion is damped, and translate this into a bound on a dissipative mutual friction-type coupling between the star's crust and core.

==> Table_BaseModel_prior.tex <==
\begin{tabular}{lll} \hhline{===}
        Parameter & Distribution &  Units\\ \hline
$\nu_0$ & $\mathcal{N}$(2.46887171470, ${7.0}{\times} 10^{\textrm{-}11}$) & Hz\\
$\dot{\nu}_0$ & $\mathcal{N}$(${\text{\textrm{-}}3.658728}{\times} 10^{\textrm{-}13}$, ${5.0}{\times} 10^{\textrm{-}19}$) & Hz/s\\
$\ddot{\nu}_0$ & $\mathcal{N}$(${8.72}{\times} 10^{\textrm{-}25}$, ${9.0}{\times} 10^{\textrm{-}27}$) & Hz/s$^{2}$\\
$\epsilon_\mathrm{p}$
 & $|\mathcal{N}$(0, ${1}{\times} 10^{\textrm{-}8}$)| &  \\
$\theta$
 & Unif(0, 0.1) & rad\\
$\chi$
 & Unif($2\pi/5$, $\pi/2$) & rad\\
$\psi_0$
 & Unif(0, $2\pi$) & rad\\
$\rho_{2}^{0}$
 & Unif(0, 0.1464) & rad\\
$\rho_{2}''$
 & $\mathcal{N}$(0, 6.83) & rad$^{\textrm{-}2}$\\
$\cos(\iota)$
 & Unif(\textrm{-}1, 1) &  \\
$\sigma_{\dot{\nu}}$
 & Unif(0, ${1}{\times} 10^{\textrm{-}15}$) & $\mathrm{s}^{\textrm{-}2}$\\
$\sigma_{W_{10}}$
 & Unif(0, 5) & ms\\
\hhline{===}
\end{tabular}


==> Table_EpsilonPoisson_posterior.tex <==
\begin{tabular}{lll} \hhline{===}
        Parameter & Median $\pm$ s.d. &  Units\\ \hline
$n$\textrm{-}$n^{\tiny\textrm{ATNF}}$ & 16.1051$\pm$0.1282 & \\
$P$\textrm{-}$P^{\tiny\textrm{ATNF}}$
 & 0.4050$\pm$${1.27}{\times} 10^{\textrm{-}11}$ & s\\
$\dot{P}$\textrm{-}$\dot{P}^{\tiny\textrm{ATNF}}$
 & ${6.0025}{\times} 10^{\textrm{-}14}$$\pm$${9.49}{\times} 10^{\textrm{-}20}$ & s\\
$\epsilon_\mathrm{p}$
 & ${9.0525}{\times} 10^{\textrm{-}9}$$\pm$${3.38}{\times} 10^{\textrm{-}11}$ &  \\
$\log_{10}(\lambda)$ & 88.7097$\pm$6.9383 & \\
$\Delta$ & ${7.3208}{\times} 10^{\textrm{-}4}$$\pm$${7.23}{\times} 10^{\textrm{-}5}$ & \\
$\theta$
 & 0.0548$\pm$0.0014 & rad\\
$\chi$
 & 1.5525$\pm$0.0008 & rad\\
$\psi_0$
 & 4.7907$\pm$0.0444 & rad\\
$\rho_{2}^{0}$
 & 0.0234$\pm$0.0004 & rad\\
$\rho_{2}''$
 & 3.5513$\pm$0.3117 & rad$^{\textrm{-}2}$\\
$\cos(\iota)$
 & ${8.0753}{\times} 10^{\textrm{-}3}$$\pm$${1.46}{\times} 10^{\textrm{-}3}$ &  \\
$\sigma_{\dot{\nu}}$
 & ${2.607}{\times} 10^{\textrm{-}16}$$\pm$${1.38}{\times} 10^{\textrm{-}17}$ & $\mathrm{s}^{\textrm{-}2}$\\
$\sigma_{W_{10}}$
 & ${1.5144}{\times} 10^{\textrm{-}3}$$\pm$0.0456 & ms\\
\hhline{===}
\end{tabular}

